Topic-Guided Self-Introduction Generation for Social Media Users

Millions of users are active on social media. To allow users to better showcase themselves and network with others, we explore the auto-generation of social media self-introduction, a short sentence outlining a user's personal interests. While most prior work profiles users with tags (e.g., ages), we investigate sentence-level self-introductions to provide a more natural and engaging way for users to know each other. Here we exploit a user's tweeting history to generate their self-introduction. The task is non-trivial because the history content may be lengthy, noisy, and exhibit various personal interests. To address this challenge, we propose a novel unified topic-guided encoder-decoder (UTGED) framework; it models latent topics to reflect salient user interest, whose topic mixture then guides encoding a user's history and topic words control decoding their self-introduction. For experiments, we collect a large-scale Twitter dataset, and extensive results show the superiority of our UTGED to the advanced encoder-decoder models without topic modeling.

==> Table/topic_words_number.tex <==
\begin{table}[t]
	 \centering
{\renewcommand{\arraystretch}{0.9}
\resizebox{0.8\columnwidth}{!}
{
	\begin{tabular}[b]{l c c c}
		\toprule
		\textbf{Words Number}        & \textbf{R-1} & \textbf{R-2} &\textbf{R-L}  \\
		\midrule
		
     	5 &   &    &    \\
      15 &   &   &   \\
            30 &   &    &   \\
            45 &   &   &    \\


	    
		\bottomrule	\end{tabular}}}
	% \vspace{-1.5em}
	\caption{
	Topic words number effects
	}
	% \vspace{-1em}
	\label{tab:topic_words_num_results}
\end{table}
